Sliced Inverse Regression Revisited: When the Number of Predictors Grows Proportionally With the Sample Size

Li (1991) introduced sliced inverse regression (SIR) as a dimension reduction method and established its theoretical properties under the assumption that the number of predictors $p$ remains fixed as the sample size $n$ tends to infinity. In this paper, we revisit the theoretical properties of SIR in the high-dimensional regime where $p/n \to \gamma \in [0,1)$, assuming normally distributed predictors and a fixed number of slices. We show that the sample SIR eigenvalues exhibit an upward bias when $\gamma>0$, that their fluctuations are governed by the Gaussian orthogonal ensemble, and that the signal eigenvalues are asymptotically normal after an appropriate bias correction. We demonstrate that Li's chi-squared test requires a scaling adjustment to achieve the nominal asymptotic size when $\gamma>0$. We further propose two additional tests that achieve the nominal asymptotic size: an exact test based on Li's test statistic and a largest-eigenvalue test. In addition, we derive closed-form limits for the accuracy of the estimated SIR directions and show that their first-order expansions in $\gamma$ agree with Li's approximation. Finally, we establish the limiting distribution of the estimated sufficient predictors for a new observation and show that, when $\gamma>0$, they contain an additional independent Gaussian noise component. Simulation studies corroborate our theoretical findings.

==> simulation/tables/tab-dhat.tex <==
\begin{tabular}{rrr ccc ccc ccc ccc}
\toprule
& & & \multicolumn{3}{c}{Li's $\chi^2$} & \multicolumn{3}{c}{corrected} & \multicolumn{3}{c}{exact} & \multicolumn{3}{c}{largest}\\
\cmidrule(lr){4-6}\cmidrule(lr){7-9}\cmidrule(lr){10-12}\cmidrule(lr){13-15}
Model & $H$ & $\gamma$ & $<$ & $=$ & $>$ & $<$ & $=$ & $>$ & $<$ & $=$ & $>$ & $<$ & $=$ & $>$\\
\midrule
1 & 5 & 0.10 & 0.000 & 0.962 & 0.038 & 0.000 & 0.947 & 0.053 & 0.000 & 0.955 & 0.045 & 0.000 & 0.934 & 0.066\\
 &  & 0.25 & 0.000 & 0.969 & 0.031 & 0.000 & 0.940 & 0.060 & 0.000 & 0.949 & 0.051 & 0.000 & 0.933 & 0.066\\
 &  & 0.50 & 0.000 & 0.992 & 0.008 & 0.000 & 0.939 & 0.061 & 0.000 & 0.951 & 0.049 & 0.000 & 0.953 & 0.047\\
 &  & 0.75 & 0.059 & 0.940 & 0.001 & 0.000 & 0.946 & 0.054 & 0.001 & 0.957 & 0.042 & 0.000 & 0.961 & 0.039\\
 & 10 & 0.10 & 0.000 & 0.954 & 0.046 & 0.000 & 0.943 & 0.057 & 0.000 & 0.951 & 0.049 & 0.000 & 0.862 & 0.138\\
 &  & 0.25 & 0.000 & 0.966 & 0.034 & 0.000 & 0.943 & 0.057 & 0.000 & 0.949 & 0.051 & 0.000 & 0.909 & 0.091\\
 &  & 0.50 & 0.000 & 0.982 & 0.018 & 0.000 & 0.940 & 0.060 & 0.000 & 0.952 & 0.048 & 0.000 & 0.949 & 0.051\\
 &  & 0.75 & 0.476 & 0.524 & 0.000 & 0.035 & 0.892 & 0.072 & 0.044 & 0.907 & 0.048 & 0.000 & 0.982 & 0.018\\
\midrule
2 & 5 & 0.10 & 0.000 & 0.963 & 0.037 & 0.000 & 0.950 & 0.050 & 0.000 & 0.957 & 0.043 & 0.000 & 0.936 & 0.064\\
 &  & 0.25 & 0.001 & 0.970 & 0.029 & 0.000 & 0.944 & 0.056 & 0.000 & 0.951 & 0.049 & 0.000 & 0.942 & 0.058\\
 &  & 0.50 & 0.208 & 0.784 & 0.007 & 0.066 & 0.888 & 0.045 & 0.080 & 0.880 & 0.040 & 0.002 & 0.959 & 0.039\\
 &  & 0.75 & 0.935 & 0.064 & 0.000 & 0.404 & 0.552 & 0.044 & 0.447 & 0.523 & 0.030 & 0.237 & 0.742 & 0.021\\
 & 10 & 0.10 & 0.000 & 0.962 & 0.038 & 0.000 & 0.945 & 0.055 & 0.000 & 0.955 & 0.045 & 0.000 & 0.899 & 0.101\\
 &  & 0.25 & 0.009 & 0.966 & 0.025 & 0.006 & 0.938 & 0.055 & 0.006 & 0.953 & 0.041 & 0.000 & 0.929 & 0.071\\
 &  & 0.50 & 0.435 & 0.556 & 0.009 & 0.180 & 0.771 & 0.049 & 0.218 & 0.750 & 0.032 & 0.000 & 0.961 & 0.039\\
 &  & 0.75 & 0.966 & 0.034 & 0.000 & 0.559 & 0.395 & 0.046 & 0.642 & 0.336 & 0.022 & 0.330 & 0.661 & 0.008\\
\bottomrule
\end{tabular}


==> simulation/tables/tab-directions.tex <==
\begin{tabular}{rrr r c ccc cc cc}
\toprule
Model & $p$ & $\gamma$ & $k$ & $\rho_k^2$ & $\hat\beta_k^T\Sigma\beta_k$ & $\hat\beta_k^T\Sigma\hat\beta_k$ & PE$_k$ & $R^2(\hat\beta_k)$ & plug-in & $R^2(\hat\beta_{1:d})$ & \eqref{eq:li51}\\
\midrule
1 & 250 & 0.25 & 1 & 0.716 & .954 (.954) & 1.03 (1.03) & .124 (.122) & .883 (.883) & .885 & .883 (.883) & .901\\
1 & 500 & 0.50 & 1 & 0.716 & .916 (.914) & 1.17 (1.17) & .341 (.338) & .716 (.716) & .720 & .716 (.716) & .802\\
1 & 750 & 0.75 & 1 & 0.716 & .879 (.878) & 1.71 (1.69) & .956 (.931) & .452 (.457) & .465 & .452 (.457) & .703\\
2 & 250 & 0.25 & 1 & 0.596 & .923 (.925) & 1.05 (1.05) & .206 (.199) & .814 (.816) & .820 & .688 (.694) & .638\\
 &  &  & 2 & 0.309 & .793 (.801) & 1.13 (1.12) & .545 (.518) & .562 (.572) & .580 &  & \\
2 & 500 & 0.50 & 1 & 0.596 & .859 (.864) & 1.26 (1.25) & .545 (.525) & .589 (.596) & .607 & .439 (.452) & .273\\
 &  &  & 2 & 0.309 & .663 (.687) & 1.56 (1.53) & 1.235 (1.155) & .288 (.309) & .328 &  & \\
2 & 1000 & 0.50 & 1 & 0.572 & .852 (.853) & 1.27 (1.27) & .571 (.566) & .571 (.572) & .574 & .404 (.407) & .029\\
 &  &  & 2 & 0.241 & .616 (.624) & 1.62 (1.61) & 1.393 (1.364) & .236 (.241) & .243 &  & \\
\bottomrule
\end{tabular}


==> simulation/tables/tab-eigen.tex <==
\begin{tabular}{rrrrr r c c c c c c}
\toprule
Model & $n$ & $p$ & $H$ & $\gamma$ & $k$ & $\rho_k^2$ & $\hat\lambda_k$ & $\ta_k$ & $\hat\rho_k^2$ & $n\,var(\hat\rho_k^2-\ta_k)$ & corr\\
\midrule
1 & 1000 & 250 & 5 & 0.25 & 1 & 0.716 & 0.789 (0.787) & 0.718 & 0.719 & 0.052 (0.054) & $\phantom{-}0.034$\\
1 & 1000 & 500 & 5 & 0.50 & 1 & 0.716 & 0.860 (0.858) & 0.719 & 0.720 & 0.161 (0.161) & $-0.029$\\
1 & 1000 & 750 & 5 & 0.75 & 1 & 0.716 & 0.931 (0.929) & 0.718 & 0.722 & 0.479 (0.483) & $\phantom{-}0.024$\\
2 & 1000 & 250 & 10 & 0.25 & 1 & 0.596 & 0.702 (0.696) & 0.601 & 0.603 & 0.109 (0.109) & $-0.021$\\
 &  &  &  &  & 2 & 0.309 & 0.486 (0.481) & 0.311 & 0.316 & 0.305 (0.319) & $-0.004$\\
2 & 1000 & 500 & 10 & 0.50 & 1 & 0.596 & 0.803 (0.798) & 0.602 & 0.607 & 0.306 (0.327) & $\phantom{-}0.006$\\
 &  &  &  &  & 2 & 0.309 & 0.664 (0.654) & 0.312 & 0.328 & 0.883 (0.956) & $-0.044$\\
2 & 2000 & 1000 & 5 & 0.50 & 1 & 0.572 & 0.787 (0.786) & 0.573 & 0.574 & 0.384 (0.366) & $\phantom{-}0.003$\\
 &  &  &  &  & 2 & 0.241 & 0.621 (0.621) & 0.240 & 0.243 & 1.188 (1.151) & $-0.042$\\
\midrule
& & & & & $t$ & & mean $L_d$ & sd $L_d$ & $q_{0.95}(L_d)$ & size & \\
\midrule
1 & 1000 & 250 & 5 & 0.25 & 3 &  & 2.09 (2.07) & 1.16 (1.09) & 4.04 (3.92) & 0.060 & \\
1 & 1000 & 500 & 5 & 0.50 & 3 &  & 2.06 (2.07) & 1.07 (1.09) & 3.80 (3.92) & 0.041 & \\
1 & 1000 & 750 & 5 & 0.75 & 3 &  & 2.03 (2.07) & 1.03 (1.09) & 3.78 (3.92) & 0.042 & \\
2 & 1000 & 250 & 10 & 0.25 & 7 &  & 4.27 (4.19) & 1.02 (0.93) & 6.04 (5.78) & 0.078 & \\
2 & 1000 & 500 & 10 & 0.50 & 7 &  & 4.03 (4.19) & 0.89 (0.93) & 5.61 (5.78) & 0.029 & \\
2 & 2000 & 1000 & 5 & 0.50 & 2 &  & 1.15 (1.25) & 1.20 (1.19) & 3.22 (3.25) & 0.048 & \\
\bottomrule
\end{tabular}


==> simulation/tables/tab-size.tex <==
\begin{tabular}{rrrr rr rrr cccc}
\toprule
& & & & \multicolumn{2}{c}{mean of $T_d$} & \multicolumn{3}{c}{$var(T_d)/(2f_d)$} & \multicolumn{4}{c}{empirical size}\\
\cmidrule(lr){5-6}\cmidrule(lr){7-9}\cmidrule(lr){10-13}
Model & $H$ & $\gamma$ & $f_d$ & MC & $\bE(T_d^*)$ & MC & exact & $1-\gamma$ & $\chi^2$ & corrected & exact & largest\\
\midrule
0 & 5 & 0.10 & 400 & 400.1 & 400.4 & 0.901 & 0.897 & 0.90 & 0.042 (0.041) & 0.048 & 0.047 & 0.082\\
 &  & 0.25 & 1000 & 1000.3 & 1001.0 & 0.806 & 0.747 & 0.75 & 0.037 (0.029) & 0.062 & 0.056 & 0.060\\
 &  & 0.50 & 2000 & 2000.9 & 2002.0 & 0.519 & 0.498 & 0.50 & 0.010 (0.010) & 0.055 & 0.051 & 0.045\\
 &  & 0.75 & 3000 & 3004.4 & 3003.0 & 0.237 & 0.249 & 0.25 & 0.000 (0.001) & 0.053 & 0.044 & 0.034\\
 & 10 & 0.10 & 900 & 901.5 & 900.9 & 0.867 & 0.893 & 0.90 & 0.045 (0.041) & 0.056 & 0.052 & 0.146\\
 &  & 0.25 & 2250 & 2253.2 & 2252.3 & 0.722 & 0.744 & 0.75 & 0.032 (0.029) & 0.057 & 0.055 & 0.089\\
 &  & 0.50 & 4500 & 4504.9 & 4504.5 & 0.491 & 0.495 & 0.50 & 0.010 (0.010) & 0.064 & 0.057 & 0.054\\
 &  & 0.75 & 6750 & 6757.3 & 6756.8 & 0.252 & 0.247 & 0.25 & 0.000 (0.001) & 0.064 & 0.056 & 0.013\\
\midrule
1 & 5 & 0.10 & 297 & 297.0 & 297.6 & 0.912 & 0.901 & 0.90 & 0.038 (0.041) & 0.053 & 0.045 & 0.066\\
 &  & 0.25 & 747 & 749.3 & 748.5 & 0.745 & 0.750 & 0.75 & 0.031 (0.029) & 0.060 & 0.051 & 0.066\\
 &  & 0.50 & 1497 & 1498.0 & 1500.0 & 0.507 & 0.500 & 0.50 & 0.008 (0.010) & 0.061 & 0.049 & 0.048\\
 &  & 0.75 & 2247 & 2251.4 & 2251.5 & 0.243 & 0.249 & 0.25 & 0.001 (0.001) & 0.053 & 0.042 & 0.040\\
 & 10 & 0.10 & 792 & 793.4 & 793.6 & 0.890 & 0.896 & 0.90 & 0.046 (0.041) & 0.057 & 0.050 & 0.138\\
 &  & 0.25 & 1992 & 1996.0 & 1996.0 & 0.769 & 0.747 & 0.75 & 0.034 (0.029) & 0.057 & 0.051 & 0.091\\
 &  & 0.50 & 3992 & 3997.2 & 4000.0 & 0.539 & 0.497 & 0.50 & 0.018 (0.010) & 0.060 & 0.048 & 0.051\\
 &  & 0.75 & 5992 & 6001.9 & 6004.0 & 0.244 & 0.248 & 0.25 & 0.000 (0.001) & 0.072 & 0.048 & 0.018\\
\midrule
2 & 5 & 0.10 & 196 & 195.5 & 196.6 & 0.891 & 0.904 & 0.90 & 0.037 (0.041) & 0.050 & 0.043 & 0.064\\
 &  & 0.25 & 496 & 497.0 & 497.5 & 0.776 & 0.754 & 0.75 & 0.029 (0.029) & 0.056 & 0.049 & 0.058\\
 &  & 0.50 & 996 & 994.8 & 999.0 & 0.497 & 0.502 & 0.50 & 0.007 (0.010) & 0.045 & 0.040 & 0.040\\
 &  & 0.75 & 1496 & 1494.4 & 1500.5 & 0.242 & 0.250 & 0.25 & 0.000 (0.001) & 0.044 & 0.030 & 0.021\\
 & 10 & 0.10 & 686 & 686.5 & 688.1 & 0.863 & 0.900 & 0.90 & 0.038 (0.041) & 0.056 & 0.045 & 0.101\\
 &  & 0.25 & 1736 & 1735.9 & 1741.2 & 0.727 & 0.750 & 0.75 & 0.025 (0.029) & 0.056 & 0.041 & 0.071\\
 &  & 0.50 & 3486 & 3487.1 & 3496.5 & 0.470 & 0.499 & 0.50 & 0.009 (0.010) & 0.049 & 0.032 & 0.040\\
 &  & 0.75 & 5236 & 5233.6 & 5251.8 & 0.256 & 0.249 & 0.25 & 0.000 (0.001) & 0.046 & 0.022 & 0.009\\
\bottomrule
\end{tabular}

